A Survey on Universal Design for Fitness Wearable Devices

Driven by the visions of Internet of Things and 5G communications, recent years have seen a paradigm shift in personal mobile devices, from smartphones towards wearable devices. Wearable devices come in many different forms targeting different application scenarios. Among these, the fitness wearable devices (FWDs) are proven to be one of the forms that intrigue the market and occupy an increasing trend in terms of the market share. Nevertheless, although the fitness wearable devices nowadays are functionally self-contained based on the advanced sensor, computation, and communicative technologies, there is still a large gap to truly satisfy the target customer group, i.e., accessible to and usable by a larger quantity of users. This fuels the research area on applying the universal design principles to fitness wearable devices. In this survey, we first present the background of FWDs and show the acceptance and adaption challenges of the corresponding user groups. We then review the universal design principle and how it and its relative approaches could be used in FWDs. Further, we collect the available FWDs that bear the universal design principles in their development circles. Last, we open up the discussion based on the surveyed literature and provide the insight of potential future work.

==> challenges.tex <==
\section{Challenges of Multipath Transmission in 5G}
\ozgu{This section is too short and not sure where to fit this. My idea was to discuss little bit the challenges of multipath in 5g after giving the background. So here the discussion should be what will be upcoming in 5g and how they will impact for example the congestion and scheduling in multipath. Something along those lines.}
TR 23.793 \cite{TR23793} is conducting study on how the 5G System (5GS) can be extended in order to support Access Traffic Steering, Switching and Splitting (ATSSS) between 3GPP and non-3GPP access networks. And such support is beneficial to the accomplishment of KPI defined in URLLC and eMBB, for two reasons:
\begin{itemize}
    \item Multipath transmission endows the connection to transparently use multiple path simultaneously thus achieving increased capacity based on concurrent transmission and high mobility based on smooth handover, mapping to the requirements from eMBB. 
    \item uRLLC targets at low latency and high reliable communication. And the high reliability part can be achieved by multipath transmission. On one side, as shown in \cite{baltrunas2016investigating}, the majority of packet loss in MBB is caused by handover. The path redunduncy adds the smooth handover functionality. On the other side, even in the non-handover scenario, the packet duplication can be used to enhance the robustness of the connection. 
\end{itemize}

Next, we will summarize the state of the art algorithms in multipath transmission and how they can help achieve eMBB and uRLLC use cases.
